Computation and Communication Co-scheduling for Multi-Task Remote Inference

In multi-task remote inference systems, an intelligent receiver (e.g., command center) performs multiple inference tasks (e.g., target detection) using data features received from several remote sources (e.g., edge devices). Key challenges to facilitating timely inference in these systems arise from (i) limited computational power of the sources to produce features from their inputs, and (ii) limited communication resources of the channels to carry simultaneous feature transmissions to the receiver. We develop a novel computation and communication co-scheduling methodology which determines feature generation and transmission scheduling to minimize inference errors subject to these resource constraints. Specifically, we formulate the co-scheduling problem as a weakly-coupled Markov decision process with Age of Information (AoI)-based timeliness gauging the inference errors. To overcome its PSPACE-hard complexity, we analyze a Lagrangian relaxation of the problem, which yields gain indices assessing the improvement in inference error for each potential feature generation-transmission scheduling action. Based on this, we develop a reoptimized maximum gain first (MGF) policy. We show that this policy is asymptotically optimal for the original problem as the number of inference tasks and the available communication and computation resources increase, provided the ratio among them remains fixed. Experiments demonstrate that reoptimized MGF obtains significant improvements over baseline policies for varying numbers of tasks, channels, and sources.

==> SchedulingPrevious.tex <==
\section{Transmission Scheduling Policy}
For any feature generation policy $f \in \mathcal F$ that satisfies the constraint \eqref{Sceduling_constraint1}, we first find a scheduling policy $g \in \mathcal G$ that minimizes the summation of the time-averaged expected inference errors of the $M$ inference tasks:
\begin{align}\label{Multi-scheduling_problem_g}
&\inf_{g \in \mathcal G}\sum_{m=1}^M  \limsup_{T\rightarrow \infty}\mathbb{E}_{(f, g)} \left[\frac{1}{T} \sum_{t=0}^{T-1} p_m(\Delta_m(t))\right], 
\\\label{Sceduling_constraint2_g}
&~\mathrm{s.t.} \sum_{m=1}^M u_{m, 2}(t)N_m \leq N, ~~t=0, 1, 2, \ldots,
\end{align}

Problem \eqref{Multi-scheduling_problem_g}-\eqref{Sceduling_constraint2_g} is a Restless Multi-armed Bandit (RMAB) problem, in which $\Delta_m(t)$ is the state of the $m$-th bandit. 
At time slot $t$, if a feature for $m$-th inference task is sent, bandit $m$ is said to be \emph{active}; otherwise, bandit $m$ is said to be \emph{passive}. 
The bandits are ``restless" because the state $\Delta_m(t)$ undergoes changes even when the $m$-th bandit is passive \cite{whittle1988restless, Tripathi2019}. It is well-known that RMAB is PSPACE-hard \cite{papadimitriou1994complexity}. We replace the per-slot channel constraints \eqref{Sceduling_constraint2_g} by a time-average expected channel constraint \eqref{changed_constraint2_g}, which produces the following relaxed problem:
\begin{align}\label{relaxed_multiple}
&\inf_{g \in \mathcal G}\sum_{m=1}^M  \limsup_{T\rightarrow \infty}\mathbb{E}_{(f, g)} \left[\frac{1}{T} \sum_{t=0}^{T-1} p_m(\Delta_m(t))\right], 
\\\label{changed_constraint2_g}
&~\mathrm{s.t.} \sum_{m=1}^M \limsup_{T \to \infty} \mathbb E_g\left[\frac{1}{T}\sum_{t=0}^{T-1} u_{m, 2}(t)N_m\right] \leq N, ~~t=0, 1, 2, \ldots.
\end{align} 
The optimal objective value of \eqref{relaxed_multiple}-\eqref{changed_constraint2_g} provides a lower bound of the optimal objective value of \eqref{Multi-scheduling_problem_g}-\eqref{Sceduling_constraint2_g}. We solve the relaxed problem \eqref{relaxed_multiple}-\eqref{changed_constraint2_g} by Lagrangian dual optimization \cite{whittle1988restless, palomar2006tutorial}. To that end, we associate a Lagrangian multiplier $\lambda \geq 0$ to the constraint \eqref{changed_constraint2_g} and get the following dual function:
\begin{align}\label{lagrangianproblem}
q(\lambda)=&\inf_{g \in \mathcal G} \sum_{m=1}^M \limsup_{T\rightarrow \infty}~\mathbb{E}_{f,g}\bigg[ \frac{1}{T} \sum_{t=0}^{T-1} \bigg(p_m(\Delta_m(t))\nonumber\\
&~~~~+ \lambda \bigg(\sum_{m=1}^M u_{m,2}(t)N_m-N\bigg)\bigg) \bigg],
\end{align}
where $\lambda \geq 0$ is also referred to as the channel occupancy or transmission cost. The problem \eqref{lagrangianproblem} can be decomposed into $M$ sub-problems. For each $m=1,2, \ldots, M$, the sub-problem associated with bandit $m$ is given by
\begin{align}\label{decoupled_problem}
&\bar p_{m, f, opt}(\lambda)\nonumber\\
&=\inf_{g_m \in \mathcal G_m} \!\!\!\limsup_{T\rightarrow \infty} \mathbb{E}_{f, g_m}\!\left[ \frac{1}{T}\!\!\sum_{t=0}^{T-1} p_m(\Delta_m(t))\!+\! \lambda u_{m, 2}(t) N_m \right],\!\!\!\!
\end{align}
where $g_m=(u_{m, 2}(0), u_{m, 2}(1), \ldots)$ is a feature sending policy for the $m$-th inference task, $\mathcal G_m$ is the set of all causal signal-ignorant feature sending policy $g_m$, and $p_{m, f, opt}(\lambda)$ is the optimal objective value of \eqref{decoupled_problem}.

\begin{theorem}\label{theoremdecoupled}
  For any policy $f \in \mathcal F$, there exists an index-based threshold policy $g^*_m=(u^*_{m, 2}(0), u^*_{m,2}(1), \ldots)$, which is optimal to \eqref{decoupled_problem}. It is optimal to request a feature for the $m$-th inference task at time slot $t$, i.e., $u^*_{m, 2}(t)=1$ if
   \begin{align}
   \gamma_m(\Delta_m(t))\geq \beta_m(\lambda),
   \end{align}
   and not to request, i.e., $u^*_{m, 2}(t)=0$, otherwise, where the index function $\gamma_m(\delta)$ is given by 
  \begin{align}\label{indexm}
\gamma_m(\delta)=\inf_{\tau \in \{1, 2, \ldots\}} \frac{1}{\tau} \sum_{k=0}^{\tau-1} \mathbb E \left [ p_m(\delta+k+1) \right],
\end{align}
and the threshold $\beta_m(\lambda)$ is 
equal to the optimal objective value of \eqref{decoupled_problem}, i.e., $\beta_m(\lambda)=p_{m, f, opt}(\lambda)$. Moreover, the threshold $\beta_m(\lambda)$ is the unique root of 
\begin{align}\label{bisectionM}
&\!\!\!\mathbb{E}\left[\sum_{t=S_{m,i}(\beta_{m}(\lambda))}^{S_{m, i+1}(\beta_{m}(\lambda))-1} p_m\big(\Delta_m(t)\big)\right]+\lambda N_m\nonumber\\
&- \beta_{m}(\lambda)~ \mathbb{E}\left[S_{m, i+1}(\beta_{m}(\lambda))-S_{m,i}(\beta_{m}(\lambda))\right]=0,
\end{align}
where $S_{m, i+1}$ is the $(i+1)$-th feature request for the $m$-th inference task, determined by
\begin{align}
&S_{m, i+1}(\beta_{m}(\lambda))\nonumber\\
&= \min_{t \in \mathbb Z}\big\{ t \geq S_{m,i}(\beta_{m}(\lambda))+1: \gamma_m(\Delta_m(t)) \geq \beta_{m}(\lambda)\big\}.
\end{align}
\end{theorem}

{\blue The optimal policy in Theorem \ref{theoremdecoupled} is similar to that in \cite[Theorem 4]{ShisherMobihoc}, yet with key distinctions. While \cite{ShisherMobihoc} assumes feature generation at each time slot $t$, our work considers feature generation under any policy $f \in \mathcal F$.  We extend the results of \cite{ShisherMobihoc} by proving that the scheduling policy in \cite{ShisherMobihoc} remains optimal even when feature generation is not constrained to every time slot.}

\subsection{Whittle Index-based Policy for \eqref{Multi-scheduling_problem_g}-\eqref{Sceduling_constraint2_g}}
The Whittle index theory only applies to RMAB problems that are indexable \cite{whittle1988restless}. Hence, we first establish the indexibility. Define $\Omega_m(\lambda)$ as the set of all states $\delta$ such that if $\Delta_m(t)=\delta$, then the optimal solution for \eqref{decoupled_problem} is to take the passive action at time $t$, i.e., $u^*_m(t)=0$. 

\begin{definition}[\textbf{Indexability}]\label{indexability}
Bandit $m$ is said to be
indexable if, as the cost $\lambda$ increases from $-\infty$ to $\infty$, the set $\Omega_m(\lambda)$ increases monotonically, i.e., $\lambda \leq \lambda_2$
implies $\Omega_m(\lambda) \subseteq \Omega_m(\lambda_2)$.
The RMAB problem \eqref{relaxed_multiple}-\eqref{changed_constraint2_g} is said to be indexable if all $M$ bandits are indexable.
\end{definition}

\begin{theorem}\label{theorem7}
The RMAB problem \eqref{relaxed_multiple}-\eqref{changed_constraint2_g} is indexable.
\end{theorem}

\begin{definition}[\textbf{Whittle index}]
Given indexability, the Whittle index $W_{m}(\delta)$ of bandit $m$ at state $\delta$ is 
\begin{align}\label{defWhittle}
W_{m}(\delta) = \inf \{\lambda \in\mathbb R: \delta \in \Omega_{m}(\lambda)\}. 
\end{align}
\end{definition}

\begin{theorem}\label{theorem8}
The Whittle index $W_m(\delta)$ of bandit $m$ is given by
\begin{align}\label{Whittle_Index}
W_{m}(\delta)=&\mathbb{E}\bigg[S_{m, i+1}(\gamma_m(\delta))-S_{m, i}(\gamma_m(\delta))\bigg]~\gamma_m(\delta)\nonumber\\
&-\mathbb E\left[\sum_{t=S_{m,i}(\gamma_m(\delta))}^{S_{m, i+1}(\gamma_m(\delta))-1} p_m(\Delta_{m}(t))\right],
\end{align}
where $\Delta_m(t)=t-S_{m, i}(\gamma_m(\delta))+b$, $\gamma_m(\delta)$ is defined in \eqref{indexm}, and $S_{m, i+1}(\gamma_m(\delta))$ is given by
\begin{align}\label{OptimalPolicyWhittle}
&S_{m, i+1}(\gamma_m(\delta))\nonumber\\
&=\min_{t \in \mathbb Z}\big\{ t \geq S_{m,i}(\gamma_m(\delta))+1: \gamma_m(\Delta_m(t)) \geq \gamma_m(\delta)\big\}.
\end{align}
\end{theorem}

{\blue Now, we are ready to state the scheduling policy for \emph{scheduler 2} that satisfies the per-time slot constraint \eqref{Sceduling_constraint2_g}. At every time slot $t$, we select $(u_{m,2}(t))_{m=1}^M$ that maximizes total Whittle indices: 

\begin{align}
&\max_{u_{m, 2}(t) \in \{0, 1\}, \forall m} \sum_{j=1}^M W_{m}(\Delta_m(t)), \\ \label{constraintagain}
&~~~~~~~\mathrm{s.t.}~~~~~~\sum_{j=1}^M u_{m, 2}(t) N_m \leq N.
\end{align}

Question: Can we prove asymptotic optimality of our scheduling policy?}

\section{Feature Generation Policy}
We denote our Whittle index-based transmission scheduling policy by $g_w \in \mathcal G$. Given transmission scheduling policy $g_w \in \mathcal G$, our goal is to find a feature processing policy $f \in \mathcal F$ that minimizes the summation of the time-averaged expected inference errors of the $M$ inference tasks:
\begin{align}\label{Multi-scheduling_problem_f}
&\inf_{f \in \mathcal F}\sum_{m=1}^M  \limsup_{T\rightarrow \infty}\mathbb{E}_{(f, g_w)} \left[\frac{1}{T} \sum_{t=0}^{T-1} p_m(\Delta_m(t))\right], 
\\\label{Sceduling_constraint2_f}
&~\mathrm{s.t.} \sum_{m=1}^M u_{m, 1}(t)C_m \leq C, ~~t=0, 1, 2, \ldots.
\end{align}

After relaxation and Lagrangian decomposition, for each feature generator $m$, we have 

\begin{align}\label{decoupled_problem_sch1}
&\bar q_{m, g_w, opt}(\mu)\nonumber\\
&=\inf_{f_m \in \mathcal F_m} \!\!\!\limsup_{T\rightarrow \infty} \mathbb{E}_{f_m, g_w}\!\left[ \frac{1}{T}\!\!\sum_{t=0}^{T-1} p_m(\Delta_m(t))\!+\! \mu~u_{m, 2}(t) C_m \right],\!\!\!\!
\end{align}
where $f_m=(u_{m, 1}(0), u_{m, 1}(1), \ldots)$ is a feature processing policy for the $m$-th inference task, $\mathcal F_m$ is the set of all causal signal-ignorant feature sending policy $f_m$, and $q_{m, g_w, opt}(\mu)$ is the optimal objective value of \eqref{decoupled_problem_sch1}.

\begin{theorem}
Given feature sending policy $g_w \in \mathcal G$, there exists an optimal policy $f^*_m=(u^*_{m, 1}(0), u^*_{m,1}(1), \ldots)$, where $u^*_{m, 1}(t)=1$ if 
\begin{align}
&Q_{m, \mu}\left((b_m(t), (\Delta_m(t))_{m=1}^M)), 1\right)\nonumber\\
&\leq Q_{m, \mu}\left((b_m(t), (\Delta_m(t))_{m=1}^M)), 0\right),
\end{align}
otherwise, $u^*_{m, 1}(t)=0$, $b_m(t)$ is the time difference between current time $t$ and the generation time of the current feature at the $m$-th buffer of the source, the action-value function $Q_{m, \mu}\left((b_m(t), (\Delta_m(t))_{m=1}^M)), a\right)$ for $a \in \{0, 1\}$ is defined as 
\begin{align}
&Q_{m, \mu}\left((b_m(t), (\Delta_m(t))_{m=1}^M)), a\right)\nonumber\\
=~&p_m(\Delta_m(t))-\bar q_{m, g_w, opt}(\mu)+ a h_{\mu}\left(1, (\Delta_m(t+1))_{m=1}^M\right)\nonumber\\
&+ (1-a) h_{\mu}\left(b_m(t)+1, (\Delta_m(t+1))_{m=1}^M\right),
\end{align}
and $\Delta_m(t+1)=1$, if $u_{m, 2}(t)=1$ under policy $g_w$; otherwise, $\Delta_{m}(t+1)=\Delta_m(t)+1$.

\end{theorem}

\subsection{Maximum Gain First Policy for \eqref{Multi-scheduling_problem_f}-\eqref{Sceduling_constraint2_f}}
\begin{definition}[\textbf{Gain index}]
The gain index $\alpha_m(b_m, (\delta_m)_{m=1}^M)$ for the $m$-th feature generation is given by
\begin{align}
\alpha_{m, \mu}(b_m, (\delta_m)_{m=1}^M)=&Q_{m, \mu}\left((b_m, (\delta_m)_{m=1}^M)), 0\right)\nonumber\\
&-Q_{m, \mu}\left((b_m, (\delta_m)_{m=1}^M)), 1\right).
\end{align}
\end{definition}

{\blue Now, we are ready to state the scheduling policy for \emph{scheduler 1} that satisfies the per-time slot constraint \eqref{Sceduling_constraint2_f}. At every time slot $t$, we select $(u_{m,1}(t))_{m=1}^M$ that maximizes total Gain indices: 

\begin{align}
&\max_{u_{m, 1}(t) \in \{0, 1\}, \forall m} \sum_{j=1}^M \alpha_{m, \mu}\left(b_m(t), (\Delta_m(t))_{m=1}^M\right), \\ \label{constraintagain}
&~~~~~~~\mathrm{s.t.}~~~~~~\sum_{j=1}^M u_{m, 1}(t) C_m \leq C.
\end{align}}

==> SpecialCase.tex <==
In the special case of non-decreasing AoI function $p_{m, j}(\delta)$, the optimal policy follows a threshold policy, which is investigated in Appendix \ref{non-decreasing}.

\section{Special Case: Non-decreasing AoI Functions}\label{non-decreasing}
In the special case of non-decreasing AoI function $p_{m, j}(\delta)$, Lemma \ref{lemma1} presents a structure of the value function $V^{\boldsymbol{\lambda}_m, \boldsymbol{\mu}}_{m, j, t}(\cdot)$. Non-decreasing AoI function $p_{m, j}(\delta)$ implies that fresh feature is always better for the $j$-th inference task of source $m$. As proved in \cite{shishertimely}, if the target and the feature sequence form a Markov chain, then the fresh feature is always better. 

\begin{lemma}\label{lemma1}
        If $p_{m, j}(\delta)$ is a non-decreasing function of AoI $\delta$, then the value function $V^{\boldsymbol{\lambda}_m, \boldsymbol{\mu}}_{m, j, t}(b, \delta)$ is non-decreasing in $(b, \delta)$ for all $t=0,1, \ldots, T$.
\end{lemma}
\begin{proof}
      See Appendix \ref{plemma1}
\end{proof}

By using Lemma \ref{lemma1}, we get Theorem \ref{theorem2}.
\begin{theorem}\label{theorem2}
    If $p_{m, j}(\delta)$ is a non-decreasing function of AoI $\delta$, then the following assertions are true:
    \begin{itemize}
        \item[(a)] If $\lambda_m=0$ and $\mu=0$,  then both $f^*_{m, j}(t)=1$ and $g^*_{m, j}(t) =1$ are optimal for all $t=0, 1, \ldots, T$.
        \item[(b)] For any $(\lambda_m, \mu)$, if both $f^*_{m, j}(t)=1$ and $g^*_{m, j}(t)=1$ are optimal when $b_{m, j}(t)=b$ and $\Delta_{m, j}(t)=\delta$, then both $f^*_{m, j}(t)=1$ and $g^*_{m, j}(t)=1$ remain optimal when $b_{m, j}(t)=b'$ and $\Delta_{m, j}(t)=\delta'$ with $(b', \delta')\geq (b, \delta)$.
         
    \end{itemize}
\end{theorem}
\begin{proof}
    See Appendix \ref{ptheorem2}.
\end{proof}

Theorem \ref{theorem2}(a) establishes that in scenarios where fresh features improve the inference accuracy and there are no costs for computational or communication, the optimal strategy is to continuously generate and transmit new features. 
%In other words, if the inference error increases as the AoI increases, and there are no costs for computational or communication, the system should always strive to provide the fresh information.

%Theorem \ref{theorem2}(a) states that if (i) fresh feature is always better for the $j$-th inference task of source $m$ and (ii) both feature generation and transmission costs are zero for source $m$ (i.e., $\lambda_m = 0$ and $\mu = 0$), then generating a new feature and transmitting a new feature are always optimal.

Theorem \ref{theorem2}(b) investigates the monotonicity property of the optimal policy for sub-problem \eqref{subproblem} when fresher features are always beneficial. It establishes that for any non-zero computation and transmission costs, if the optimal action at time $t$ is to compute and transmit a new feature when the state is $(b_{m, j}(t), \Delta_{m, j}(t)) = (b, \delta)$, then this action remains optimal for any state $(b', \delta')$ where $b' \ge b$ and $\delta' \ge \delta$.

\section{Proof of Lemma \ref{lemma1}}\label{plemma1}
To prove Lemma \ref{lemma1}, it suffices to show that the value function $V_{t}(b, \delta)$ (where we omit superscripts and subscripts for brevity) satisfies:

\begin{align}\label{l1}
V_{t}(b, \delta) &\leq V_{t}(b, \delta+1), \\ \label{l2}
V_{t}(b, \delta) &\leq V_{t}(b+1, \delta),  \\ \label{l3}
V_{t}(b, \delta) &\leq V_{t}(b+1, \delta+1). \\
\end{align}

\noindent Case (t = T): Since $p_{m,j}(\delta)$ is non-decreasing in $\delta$ and the terminal value $V_{T+1}(b,\delta) = 0$, we have:
\begin{align}
    V_{T}(b, \delta) &= p_{m, j}(\delta)=V_{T}(b+1, \delta),\\
    &\leq  p_{m, j}(\delta+1)
    =V_{T}(b, \delta+1),\\
    &=V_{T}(b+1, \delta+1),
\end{align}
establishing \eqref{l1}-\eqref{l3} for $t = T$.

\noindent Inductive Step: Assume \eqref{l1}-\eqref{l3} hold for $t = K + 1$.  Then, using the value function update \eqref{optimalsubpolicy} and the monotonicity of $p_{m,j}(\delta)$, we have:
\begin{align}\label{lp1}
    &V_{K}(b, \delta)\nonumber\\
    &= p_{m, j}(\delta)\nonumber\\
    &+\gamma \min\{V_{K+1}(b+1, \delta+1), \lambda_m+V_{K+1}(1, \delta+1),\nonumber\\
    &~~~\mu+V_{K+1}(b+1, 1), \lambda_m+\mu+V_{K+1}(1, 1)\}\nonumber\\
    &\leq  p_{m, j}(\delta+1)\nonumber\\
    &+\gamma \min\{V_{K+1}(b+1, \delta+2), \lambda_m+V_{K+1}(1, \delta+2),\nonumber\\
    &~~~\mu+V_{K+1}(b+1, 1), \lambda_m+\mu+V_{K+1}(1, 1)\}\nonumber\\
    &=V_{K}(b, \delta+1).
\end{align}
Similarly, we can show 
\begin{align}
    V_{K}(b, \delta) \leq V_{K}(b, \delta+1)
    \leq V_{K}(b+1, \delta+1).
\end{align}
Thus, \eqref{l1}-\eqref{l3} hold for $t = K$.

By induction, we conclude that \eqref{l1}-\eqref{l3} hold for all $t$. This concludes the proof.

%Moreover, if \eqref{l1}-\eqref{l3} are true for any $t=K+1$, then we have 
%\begin{align}\label{lp2}
 %   &V_{K}(b, \delta)\nonumber\\
  %  &= p_{m, j}(\delta)\nonumber\\
  %  &+\gamma \min\{V_{K+1}(b+1, \delta+1), \lambda_m+V_{K+1}(1, \delta+1),\nonumber\\
  %  &~~~\mu+V_{K+1}(b+1, 1), \lambda_m+\mu+V_{K+1}(1, 1)\}\nonumber\\
   % &\leq  p_{m, j}(\delta+1)\nonumber\\
   % &+\gamma \min\{V_{K+1}(b+2, \delta+1), \lambda_m+V_{K+1}(1, \delta+1),\nonumber\\
   % &~~~\mu+V_{K+1}(b+2, 1), \lambda_m+\mu+V_{K+1}(1, 1)\}\nonumber\\
    %&=V_{K}(b+1, \delta).
%\end{align}
%From \eqref{lp1} and \eqref{lp2}, we get that if \eqref{l1}-\eqref{l3} are true for any $t=K+1$, we have 
%\begin{align}\label{lp3}
  %  V_{K}(b, \delta)\leq V_{K}(b+1, \delta+1).
%\end{align}
%From \eqref{lp1}-\eqref{lp3}, by using mathematical induction, we can say that \eqref{l1}-\eqref{l3} hold true for all $t$. This concludes the proof.

\section{Proof of Theorem \ref{theorem2}}\label{ptheorem2}
Part (a): By Lemma \ref{lemma1}, the value function $V^{\lambda_m, \mu}_{m, j, t+1}(b, \delta)$ is non-decreasing in both $b$ and $\delta$. Therefore, $V^{\lambda_m, \mu}_{m, j, t+1}(1, 1)$ is the minimum value over all $b \geq 1$ and $\delta \geq 1$ for all $t$. When $\lambda_m = 0$ and $\mu = 0$ (no computation or transmission costs). For this case, the Bellman equation \eqref{optimalsubpolicy} implies that the optimal policy is to always choose the action $(a_1, a_2) = (1, 1)$, which corresponds to computing and transmitting the feature at every time slot, i.e., $f^*_{m, j}(t) =1,  g^*_{m, j}(t) = 1$.

Part (b): If $f^*_{m, j}(t) = 1$ and $g^*_{m, j}(t) = 1$ is optimal for state $(b, \delta)$, then the Bellman optimality equation \eqref{optimalsubpolicy} implies:
\begin{align}\label{t2}
    &\lambda_m+\mu+\gamma V^{\lambda_m, \mu}_{m, j, t+1}(1, 1)\nonumber\\
    \leq &\min\bigg\{\gamma V^{\lambda_m, \mu}_{m, j, t+1}(b+1, \delta+1),\nonumber\\ &\lambda_m+\gamma V^{\lambda_m, \mu}_{m, j, t+1}(1, \delta+1), \mu+\gamma V^{\lambda_m, \mu}_{m, j, t+1}(b+1, 1)\bigg\}.
\end{align}
Now, by Lemma \ref{lemma1}, the value function is non-decreasing in both arguments. Therefore, for all $(b', \delta') \geq (b, \delta)$, we have the same inequalities as above but with $(b', \delta')$ instead of $(b, \delta)$. This means that the optimal policy is also to compute and transmit for all states $(b', \delta') \geq (b, \delta)$. This completes that proof.


